U-Net for MAV-based Penstock Inspection: an Investigation of Focal Loss in Multi-class Segmentation for Corrosion Identification

Periodical inspection and maintenance of critical infrastructure such as dams, penstocks, and locks are of significant importance to prevent catastrophic failures. Conventional manual inspection methods require inspectors to climb along a penstock to spot corrosion, rust and crack formation which is unsafe, labor-intensive, and requires intensive training. This work presents an alternative approach using a Micro Aerial Vehicle (MAV) that autonomously flies to collect imagery which is then fed into a pretrained deep-learning model to identify corrosion. Our simplified U-Net trained with less than 40 image samples can do inference at 12 fps on a single GPU. We analyze different loss functions to solve the class imbalance problem, followed by a discussion on choosing proper metrics and weights for object classes. Results obtained with the dataset collected from Center Hill Dam, TN show that focal loss function, combined with a proper set of class weights yield better segmentation results than the base loss, Softmax cross entropy. Our method can be used in combination with planning algorithm to offer a complete, safe and cost-efficient solution to autonomous infrastructure inspection.

==> tex/introduction.tex <==
\section{Introduction}
Regular inspection of infrastructures such as water/gas penstocks, subway tunnels, and bridges is indispensable since any damage or failure during our operation could cause deadly and extremely expensive costs. Recent bridge collapse in Italy has caused more than thirty deaths, raising a global warning on regular checking and maintaining millions of aging infrastructures worldwide. 

Traditional methods of inspection rely on manual sensing and vision monitoring which are extremely expensive, tedious and can be dangerous. For instance, inspecting one bridge takes roughly $2.5$ days for one profesional inspector \footnote{https://www.nytimes.com/1983/06/29/nyregion/how-bridges-are-inspected-and-what-is-being-done-to-make-them-safer.html}. To inspect every bridge in Connecticut state (the U.S.) once every twelve months, the current full-time team have to double in size. Thus, traditional methods are not an appropriate solution at the global scale. 

Taking these concerns, automated procedures have been proposed such as using micro aerial vehicles (MAVs) to capture photos of the infrastructures and then utilizing computer vision techniques to to achieve surveying. 
For example, Laing O'Rourke, a construction company, started using a surveying drone for their crossrail project\footnote{https://www.expouav.com/news/latest/using-drone-technology-construction-tunnel-environment/}, Sa et. al~\cite{sa2015outdoor} develop a high-speed vision system to inspect poles. 

\begin{figure}[t!]
  \vspace{3mm}
  \centering
  \includegraphics[width=\linewidth]{intro_images/drone_and_flight.png}
\caption{The UAV platform and a snapshort of its flight inside the penstock. Light is omitted from the unique source - UAV's onboard LED system}.
\label{fig:drone}
\vspace{-6mm}
\end{figure}

% https://www.expouav.com/news/latest/using-drone-technology-construction-tunnel-environment/
% Since MAVs are becoming cheaper and easier to use, we can now easily send our sensing tools into otherwise inaccessible areas. This  the breakthroughs in deeplearning-powered computer vision techniques.  factors have help extend the research horizon in field robotics, bringing us closer to automated inspection. 

This work attempts to put a milestone into making automated, cheaper and safer inspection in subterrain fields in which a large portion of civilian activities are operating, from penstocks in electricity plants to tunnels in subway systems and water absorption systems. 

To this end, We propose a data-driven method to automatically identify the corroded spots on the internal surface of the penstock from the captured images.
Fig.~\ref{fig:intro_image} shows an example where corroded spots are labeled in pink color. These spots are regions on the penstock surface which is exposed to the environment and corroded after its coating is faded away. 

Our simplified U-net can be trained on a small training set of less than $40$ image samples to detect corroded spots at the speed of $12$ $fps$ on full-size images ($1024 \times 1280$). This enables to do real-time inspection using a UAV with high image resolution.  

We discuss the class imbalance problem and the choice of different loss functions to mitigate this problem. 

We generalize the usage of focal loss function in a multi-class segmentation problem. 

We analyze different metrics to demonstrate the importance of choosing a proper metrics to evaluate the performance of the learned models.  

Our empirical experiments show that the focal loss function, associated with a proper set of class weights can improve the segmentation results and discuss the effect of the class weight on the performance of the weighted focal loss. 

Our paper is organized as follows. Section~\ref{sec:related_work} relates our work to the literature. Section~\ref{sec:dataset} briefly describe the data collection and preprocessing. After giving the problem description in Section~\ref{sec:problem}, we discuss the class imbalance problem alongside with loss functions to deal with it. Section~\ref{sec:training} describes our network as well as the training strategy, and the selection of hyper-parameters. The results that compare the performance of different loss functions as well as the effect of class weights on weighted focal loss are described in section~\ref{sec:evaluation}. Section~\ref{sec:conclusions} sums up our work with limitations and future works.  

% \begin{figure}[t]
%   \vspace{2mm}
%   \centering
% \begin{subfigure}{.48\linewidth}
%   \centering
%   \includegraphics[width=3.5cm,height=2.5cm]{intro_images/drone.jpg} 
% \end{subfigure}   
% \begin{subfigure}{.48\linewidth}
% 	\centering
%     \includegraphics[width=3.5cm, height=2.5cm]{intro_images/drone_flight.jpg}
% \end{subfigure}   
% \caption{The UAV platform and a snapshort of its flight inside the penstock. Light is omitted from the unique source - UAV's onboard LED system}.
% \label{fig:drone}
% \vspace{-5mm}
% \end{figure}






% We also raise a caution over using the focal loss. Our experiments also show that focal loss could also harm the performance without carefully selection of class weights since it may intensively focuses on "hard samples" giving less training signal to the "easy" but may "important" samples. 



==> tex/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\noindent \textbf{Deep Learning for field visual inspection}\\
There have been a huge interest in using unmanned aerial vehicles (UAVs) and deep learning techniques to inspect infrastructures. For example, authors in~\cite{lee2018diagnosis, duque2018synthesis, gopalakrishnan2018crack} develop UAV systems and algorithms to detect cracks on the surface of infrastructures. Unlike our work, these use deep networks to classify the whole image or a proposed region on the image (with predefined scales) as crack or non-crack. These techniques face a challenge in applying to our problem since the corroded spots in our images highly varies in size and appearance. 

Deep learning techniques have also been applied to a wide range of object detection applications such as detecting pedestrians~\cite{aguilar2017pedestrian, shao2018using}, vehicles~\cite{breckon2009autonomous, yang2018vehicle} 
or both~\cite{gaszczak2011real}, serving as an excellent alternative to traditional traffic monitoring and management methods.  

Wildlife monitoring is also an important subject of visual inspection techniques~\cite{aniceto2018monitoring, seymour2017automated, oishi2018animal}. 

In agriculture, deep-learning-powered image segmentation has recently achieved a lot of successes into agricultural tasks such as fruit counting~\cite{chen2017counting, zhuang2018detection, lu2017non, roy2018vision, bargoti2017deep, bargoti2017image}, and plant inspection~\cite{wang2018machine}. 

Compared to these pieces of work, there are more challenges in our visual inspection due to the imperfect lighting condition as well as the brightness noise caused by the flowing dust exposed to the LED during the flight. To the best of our knowledge, this work is the first attempt to apply deep neural networks into such environment. 


\noindent \textbf{Small training dataset} \\
For supervised learning tasks like image segmentation, training data is crucial and deep neural networks is known to require massive data samples to train. Nevertheless, in robotics and medical problems, the amount of training data is often limited due to the expense of the data collection process. To mitigate this problem, several solutions have been proposed such as generating synthetic data~\cite{georgakis2017synthesizing}, doing data augmentation~\cite{chen2018deeplab}, using transfer learning~\cite{romera2018train}, and designing data-efficient approaches, to name a few. 

A well-known success in designing data-efficient deep neural networks is U-net~\cite{ronneberger2015u} which won the
Cell Tracking Challenge at ISBI 2015\footnote{http://www.celltrackingchallenge.net/} and is capable to train on as few as $30$ data samples. Indeed, our network is a simplified version of U-net. 

Other works in biomedical imaging related to our segmentation task are ~\cite{guerrero2018multiclass, novikov2018fully}. However, they focus more into instance segmentation which attempts to separate, for example, individual biological cells, from each other. Their segmentation is also less challengs, since the lighting condition is easier to control, leading to a more distinguishable foreground's appearance.    
Unlike these biomedical and infrastructure inspection works, our images suffer from imperfect lighting condition with high exposure on reflective areas, low exposure under non-reflective areas, not to mention dust noise. In addition, the corroded spots are also highly nonhomogeneous in appearance and size, making the segmentation challenging. 


\noindent \textbf{Class imbalance} \\ 
Despite its comprehensive literature in classical machine learning, class imbalance has not attracted significant attention in the context of deep learning. There are very few works that concern this problem. For example, Buda et. al~\cite{buda2018systematic} provide a systematic investigation on class imbalance in deep learning but their solutions focus on redistribute the frequency of classes in the training dataset using sampling, two-phase training, and thresholding approaches rather than loss functions like us. Authors in~\cite{lin2018focal} propose a focal loss as an alternative to sampling methods. However, it is meant to solve the detection problem. In this study, we extend the horizon of its potential usage by investigating its effect in a multi-class segmentation problem. 








